Renewable Energy-Aware Information-Centric Networking

The ICT industry today is placed as one of the major consumers of energy, where recent reports have also shown that the industry is a major contributor to global carbon emissions. While renewable energy-aware data centers have been proposed, these solutions have certain limitations. The primary limitation is due to the design of data centers which focus on large-size facilities located in selected locations. This paper addresses this problem, by utilizing in-network caching with each router having storage and being powered by renewable energy sources (wind and solar). Besides placing contents closer to end users, utilizing in-network caching could potentially increase probability of capturing renewable energy in diverse geographical locations. Our proposed solution is dual- layered: on the first layer a distributed gradient-based routing protocol is used to discover the paths along routers that are powered by the highest renewable energy, and on the second layer, a caching mechanism will pull the contents from the data centre and place them on routers of the paths that are discovered by our routing protocol. Through our experiments on a testbed utilizing real meteorological data, our proposed solution has demonstrated increased quantity of renewable energy consumption, while reducing the workload on the data centers.

==> summary.tex <==
The results from our experimentation has shown that CCN is a viable approach towards improving renewable energy awareness in underlying communication networks. 
The results of the experimentation has demonstrated the following key points for our proposed solution:
\begin{itemize}
\item The \rePGBR{} routing protocol can adaptively cope with changing weather patterns to discover renewable energy aware paths, and at the same time is flexible enough to be 
integrated with different caching strategies (ALL, Cachedbit, NbSC).
\item Trade-off exists between enhancing caching performance and favoring more renewable energy aware paths.
\item Different seasons will have an impact on the routing performance, which in turn can be compensated with a caching strategy.
\item Brown energy savings can be achieved when we power down unused routers, while remaining routers that are used for caching are powered by renewable energy.
\end{itemize}

==> windSolarMap.tex <==
\begin{figure}[!t]
  \subfloat[Wind speed]{\includegraphics[width=0.5\linewidth]{usaAnnualWindSpeed}%
    \label{fig:windSpeed}}
  \hfill
  \subfloat[GHI]{\includegraphics[width=0.5\linewidth]{usaAnnualGHI}%
    \label{fig:ghi}}
  \caption{Average annual wind speed and Global Horizontal Irradiance in USA.}
  \label{fig:usaWeather}
\end{figure}

We use publicly available data from the National Renewable Energy Laboratory~\cite{nrel} to estimate the availability of wind and solar power in different parts of the U.S. 
Below we describe our weather data and present the methodology used to convert the meteorological wind and solar data, to power.

\subsection{Wind energy profile}
\label{sec:wind}

\figurename{ \ref{fig:windSpeed}} shows a simplified version of the
annual wind speed in the U.S.
The darker zones have an
average wind speed between $4$ - $6~m/s$, the average wind speed for
the medium zones are between $6$ - $8~m/s$, and in the brighter zone,
the average speed is greater than $8~m/s$.

We consider two wind turbines produced by the Huaying
company~\cite{windTurbineGenerator}. The two models are ``HY30-AD11''
which is a \kW{30} wind turbine, and a smaller model ``HY5-AD5.6'' which
produces energy up to \kW{5.4} (the larger turbine has a similar size
to the turbine investigated in \cite{Liu_Lin_Wierman_Low_Andrew_2011}.)

\figurename{ \ref{fig:windToPower}} presents a plot showing the
relationship of wind speed to generated power that can be achieved by
the two different turbines. As we can see, six \kW{5} wind turbines
produce more power than a single \kW{30} turbine at a low wind speed
(e.g. at $6~m/s$, the ratio is 2.9). However, the type of turbines could be decided on the space restrictions and the cost of the infrastructure.oring the use of multiple 5~kW wind turbines.

\begin{figure}[!t]
  \centering
  \subfloat[Wind speed to power conversion]{\label{fig:windToPower}\includegraphics[width=.5\linewidth]{windToPower}}
  \subfloat[Optimal mix distribution]{\label{fig:diffDistrib}\includegraphics[width=.5\linewidth]{diffDistribution_5kw_30kw}}
 \caption{Wind energy profile for different turbine types (\kW{5} and \kW{30}), as well as distribution of routers with optimal ratio of wind and solar energy sources.}
 \label{fig:impact}
\end{figure}

\subsection{Solar energy profile}
\label{sec:solar}

The Global Horizontal Irradiance (GHI) is used to estimate how much
power could be generated by photovoltaic solar panels. A \kW{4} photovoltaic solar panel that is needed to produce \kW{4} of power,
will require a GHI of $1000~W/m^2$. As shown in
\figurename {\ref{fig:ghi}}, the GHI is usually stronger in the south
west of the U.S. For example, in the brigther zone (very high GHI), the estimated
energy is greater than $6000~kWh$, while the estimated energy is only $3000~kWh$ in the zone with the lowest GHI.
